An Energy-aware Mutation Testing Framework for EAST-ADL Architectural Models

Early design artifacts of embedded systems, such as architectural models, represent convenient abstractions for reasoning about a system's structure and functionality. One such example is the Electronic Architecture and Software Tools-Architecture Description Language (EAST-ADL), a domain-specific architectural language that targets the automotive industry. EAST-ADL is used to represent both hardware and software elements, as well as related extra-functional information (e.g., timing properties, triggering information, resource consumption). Testing architectural models is an important activity in engineering large-scale industrial systems, which sparks a growing research interest. The main contributions of this paper are: (i) an approach for creating energy-related mutants for EAST-ADL architectural models, (ii) a method for overcoming the equivalent mutant problem (i.e., the problem of finding a test case which can distinguish the observable behavior of a mutant from the original one), (iii) a test generation approach based on UPPAAL Statistical Model Checker (SMC), and (iv) a test selection criteria based on mutation analysis using our MATS tool.

==> removing-mutant-models.tex <==
%Equivalent mutants are detected using an SMT-solving approach and removed from the set of \east} mutated models.
%The set of generated mutants can be processed such that the mutants who are equivalent to the original model are removed. For this purpose, we define the criteria for detecting mutants equivalent to the original model and propose a technique which can automatically perform the equivalence checking.

